Learning to Optimize Join Queries With Deep Reinforcement Learning

Exhaustive enumeration of all possible join orders is often avoided, and most optimizers leverage heuristics to prune the search space. The design and implementation of heuristics are well-understood when the cost model is roughly linear, and we find that these heuristics can be significantly suboptimal when there are non-linearities in cost. Ideally, instead of a fixed heuristic, we would want a strategy to guide the search space in a more data-driven way---tailoring the search to a specific dataset and query workload. Recognizing the link between classical Dynamic Programming enumeration methods and recent results in Reinforcement Learning (RL), we propose a new method for learning optimized join search strategies. We present our RL-based DQ optimizer, which currently optimizes select-project-join blocks. We implement three versions of DQ to illustrate the ease of integration into existing DBMSes: (1) A version built on top of Apache Calcite, (2) a version integrated into PostgreSQL, and (3) a version integrated into SparkSQL. Our extensive evaluation shows that DQ achieves plans with optimization costs and query execution times competitive with the native query optimizer in each system, but can execute significantly faster after learning (often by orders of magnitude).

==> generalization.tex <==
\section{A General Framework: Related Work}
The formulation of join optimization as a searching for sequence of graph contractions allows us to pose many common algorithms in a single unified framework. A \emph{greedy} solution to this problem is to optimize each $c_i$ independently. The algorithm proceeds as follows: (1) start with the query graph, (2) find the lowest cost contraction, (3) update the query graph and repeat. This greedy algorithm has a computational complexity of $O(|V|^3)$, and is described in \cite{d}.

The greedy algorithm, of course, does not consider how local decision might affect future costs. To find a globally optimal solution one must consider the long term value of a decision. Classical sequential decision making theory formalizes this concept with the characterization of the cost-to-go function.



\subsection{Existing Enumeration Algorithms}
This Q-function formulation gives us a way to describe many different join enumeration methods, heuristics, and robustness techniques in the same mathematical framework. We can think of it as an estimation problem where the optimizer first has to construct an estimate of the Q function $\hat{Q} \approx Q$ whether through enumeration, trial execution, heuristics, or all of the above. Then, there is a selection phase where $\hat{Q}$ is realized into a join plan. In some algorithms, these two phases are not explicit and happen simultaneously but conceptually this is the process for optimal join ordering. Many common join optimization algorithms can be interpreted as manipulating different parts of the Q function for either more efficient/robust estimation or more efficient optimization.

\vspace{0.25em} \noindent \textbf{Greedy Join Enumeration: } A greedy join enumeration strategy can be thought of as using the $\hat{Q} = J$ as an approximation for the Q-function.

\vspace{0.25em} \noindent \textbf{IK-KBZ: } For acyclic query graphs (common in star schemas), a polynomial time enumeration algorithm was proposed called IK-KBZ~\cite{?}. The informal insight is that for chain-structured query graphs and linear cost functions, finding the optimal join plan reduces to sorting the chain by ``rank'' (how much it increases or reduces the size of the input relation in a left join). This basic algorithm can be recursively applied to tree-structured query graphs where branches are converted into chains when possible and then merged. 

One can interpret this algorithm as restrictions on the structure of the Q function. First, this procedure will only produce left-deep plans. This is equivalent to saying that for $t>1$ every contraction $c(u,v)$, $v$ must be a single relation, or alternatively $\hat{Q}(G,c) = \infty$. This restriction means that the $\hat{Q}(G,c)$ is linear in the cardinality of $v$ independent of what relations are on the left. Thus, the Q-Function in this class of problems essentially ranks all single relations by how much they increase the cardinality of a left-deep chain. 

\vspace{0.25em} \noindent \textbf{Cost-Space Linearization: } Many of the ideas in IK-KBZ are useful as heuristics even if the assumptions are not satisfied~\cite{?}. This can be thought of as approximating the true Q-function with a $\hat{Q}$ that is easier to construct.

\vspace{0.25em} \noindent \textbf{System R: } Similar to IK-KBZ, but applicable to all queries the classic System R optimizer restricts the plan space to left-deep plans and avoiding Cartesian products. As before, one can think of this as, $\hat{Q}(G, c) = \infty$ for any contraction that creates a structure that is not a chain. Similarly, avoiding Cartesian products means that any contraction that is not along an edge is assumed to have a $\hat{Q}(G,c) = \infty$. However, the System R optimizer exactly calculates the Q function for all other plans.

\vspace{0.25em} \noindent \textbf{QuickPick and other Randomized Algorithms: } Random sampling based join enumeration can also be expressed in this framework, where join plans are initially sampled with a $\hat{Q}$ that is random. Then, the true cost of each sample is evaluate and the best is selected. 

\vspace{0.25em} \noindent \textbf{Summary: } We tend to think about join enumeration algorithms as combinatorial. However, thinking about the Q-Function gives us an functional perspective on the problem--namely it is fundamentally a problem of data collection (through enumeration) and function approximation (to construct the optimal sequence).  

\subsection{Inaccurate Cost Models}
All of the previously presented algorithm assume that the optimizer's internal cost model is accurate. In practice, even with exhaustive enumeration $\hat{Q}$ always approximates a true $Q^*$ that represents the real query execution performance. Several techniques have been proposed to ``correct'' the cost model based on feedback from execution~\cite{?}. Similarly, there is also a well-studied literature on robust query optimization~\cite{?} to avoid decisions that are sensitive to poor cost estimates. These approaches require careful modeling of the sources of uncertainty and sometimes only work for certain cost models (e.g., Least-Expected Cost optimization works best with linearized costs). 

Traditionally, the community has divorced the issues of enumeration and cost modeling. This paper argues that they are fundamentally a form of Q-Function approximation. Enumeration strategies place restrictions on the type of Q-function one is allowed to construct, adaptive techniques leverage feedback to correct systematic errors in the Q-function, and robust techniques try to account for uncertainty in the estimates.







==> intro-Oct19.tex <==
\section{Introduction}\label{intro}\sloppy
Join order optimization is a core component of almost all query optimizers. 
While the first approaches were proposed more than 40 years ago~\citep{selinger1979access}, the problem continues to be an active area of research~\citep{trummer2017solving,neumann2018adaptive,marcus2018deep}.
One reason for the perennial interest in the problem is its combinatorial complexity, which leads to the use of heuristic solutions in practice (e.g., the ubiquitous left-deep heuristic).
These heuristics can have weak spots leading to very suboptimal plans.
Database administrators often hand-optimize these corner cases by creating views to force certain query plans and/or tuning optimizer parameters.

In light of the recent advances in machine learning and AI, replacing programmed heuristics with learned ones is a new trend in join optimization research~\citep{marcus2018towards,kipf2018learned, ortiz2018learning,marcus2018deep}. 
Likewise, this paper explores the problem of synthesizing dataset-specific join search strategies using machine learning.
We assume a fixed cost model and plan space, and focus on optimal ways to search over the space of possible join plans.
The main idea is to learn from the results of previous planning instances and avoid search branches that were previously observed to be suboptimal.

Join order optimization is particularly interesting from a machine learning perspective because it has a well-known sequential structure that even classical join optimization algorithms exploit (e.g., Sellinger's dynamic program~\citep{selinger1979access}).
This is exactly the same problem structure, called a Markov Decision Process, that underpins stochastic sequential decision making problems in reinforcement learning (RL)~\citep{sutton1998reinforcement}. 
The main insight of this paper is that classical dynamic programming solutions to join optimization are, in a sense, degenerate RL algorithms.

To understand the connection, let us consider the classical ``bottom up'' dynamic programming solution to join ordering.
The principle of optimality leads to an algorithm that incrementally builds a plan from optimal subplans of size two, size three, and so on.
The algorithm re-uses previously enumerated subplans through exact memoization in a lookup table, and uses this table to construct a sequence of 1-step optimal decisions.
RL views this table as a model: the algorithm has access to a data structure that summarizes the results of previous enumerations and makes a future decision using this data structure.
So instead of exact memorization, a family of RL algorithms called Q-Learning poses the dynamic programming steps as a generalized prediction problem: given the costs of previously enumerated subplans, which 1-step decision is most likely optimal?
Concretely, this corresponds to setting up a regression problem between the decision to join a particular pair of relations and the observed benefit of making that decision in past data (impact on the final cost of the entire query plan).
This formulation is particularly compelling if a single model can capture predictions for an entire workload, thus sharing learned experiences across planning instances.

Casting join ordering as an RL problem sheds light on an entire spectrum of approaches spanning from pure classical enumeration to pure learning and different ways of leveraging past planning experience.
This paper demonstrates that this connection is not simply theoretical, and can actually lead to orders of magnitude faster planning in operational systems today.
We present an RL-based optimizer, called \sys, that does ordering and physical operator selection. 
In the initial implementation, we assume a read-only database and a fixed schema.
\sys observes the planning results of previously executed queries and trains an RL model to improve future search instances.
While RL algorithms are notoriously inefficient in terms of training data, \sys exploits the optimal subplan structure present in most join optimizers.
From a single query, not only is the final plan and its total cost a training example, but all of its subplans as well and their associated costs as well. 
A relatively small number of queries generates a vast amount of examples from which \sys can learn a search strategy.

We implement three versions of \sys to illustrate the ease of integration into existing DBMSes: (1) A version built on top of Apache Calcite~\citep{calcite}, (2) a version integrated in the Postgres SQL query optimizer, and (3) a version integrated into Spark SQL.
The two deployments into existing systems (2) and (3) each required less than 300 LoC and training data could be collected through the normal operation of the DBMS.
We present experimental results on two benchmark datasets and workloads: Join Order Benchmark (JOB)~\citep{leis2015good} and TPC-DS~\citep{tpcds}.
In our experiments, we are restricted to optimizing foreign-key joins due to the schemas of the experimental workloads, and discuss at the end how \sys could be applied to more general join queries.
We observe significant speedups in planning times (up-to > 200x) while essentially matching the execution times of optimal plans found through their enumeration-based native optimizers.
We also show that these speedups can facilitate broadening the plan space (e.g., to bushy plans) leading to improved query execution times as well. 
\sys is particularly useful over cost models with significant non-linearities (such as memory limits or materialization).  On two simulated cost models with significant non-linearities \sys improves on the next best heuristic over a set of 6 baselines by $1.7\times$ and $3\times$. 

This paper does not argue an application of RL to join optimization, but rather the insight that classical join optimization is deeply linked to the Q-Learning family of RL algorithms.
The link allows RL to be applied efficiently to join order optimization problems.
In particular, experiments suggest that \sys does not suffer as severe of a cold start problem endemic to existing learning-based join work where the authors report \textbf{tens of thousands} of training queries for each benchmark dataset~\citep{kipf2018learned, ortiz2018learning,marcus2018deep}, whereas, \sys requires hundreds of training queries in our experiments.
This is fundamentally because the Q-Learning algorithm leverages optimal substructures during training in contrast to other recent work like~\citep{marcus2018deep}.
We believe that addressing such data efficiency problems is the first step towards an ultimate vision of a DBMS that learns to optimize queries on its own.


==> reduction_factor_learning.tex <==
\section{Reduction factor learning}

Classical approaches to reduction factor estimation include (1) histograms and
heuristics-based analytical formulae, and (2) applying the predicate under
estimation to sampled data, among others.  In this section we explore the use of
learning in reduction factor estimation.  We train a neural network to learn the
underlying data distributions of a pre-generated database, and evaluate the
network on unseen, randomly selections that query the same database.

To gather training data, we randomly generate a database of several relations,
as well as random queries each consisting of one predicate of the form ``R.attr
$\langle$op$\rangle$ literal''.  For numeric columns, the operands are $\{=,
\neq, >, \geq, <, \leq\}$, whereas for string columns we restrict them to
equality and inequalities.  Each attribute's values are drawn from a weighted
Gaussian.

To featurize each selection, we similarly use 1-hot encodings of the participant
attribute and of the operand.  Numeric literals are then directly included in
the feature vector, whereas for strings, we embed ``hash(string\_literal) \% B''
where $B$ is a parameter controlling the number of hash buckets.  The labels are
the true reduction factors by executing the queries on the generated database.

A fully-connected neural network is used\footnote{Two hidden layers, 256 units
each, with ReLU activation.}, which is trained by stochastic gradient descent.

{\bf Evaluation.}  We compare the neural net to a simple linear regressor.  We
train on a database of 5 relations, a total of 21 attributes; the train and test
sets include 1000 and 2000 queries, respectively. We found that the fitted
linear regressor has a mean-squared-error of $\approx 84$, while the neural
network is able to achieve an L1 loss of $< 1$, approximating the true reduction
factors with minimal error.  \reminder {TODO(zongheng): they need to be on the
same scale. }

